LayoutCopilot: An LLM-powered Multi-agent Collaborative Framework for Interactive Analog Layout Design

Analog layout design heavily involves interactive processes between humans and design tools. Electronic Design Automation (EDA) tools for this task are usually designed to use scripting commands or visualized buttons for manipulation, especially for interactive automation functionalities, which have a steep learning curve and cumbersome user experience, making a notable barrier to designers' adoption. Aiming to address such a usability issue, this paper introduces LayoutCopilot, a pioneering multi-agent collaborative framework powered by Large Language Models (LLMs) for interactive analog layout design. LayoutCopilot simplifies human-tool interaction by converting natural language instructions into executable script commands, and it interprets high-level design intents into actionable suggestions, significantly streamlining the design process. Experimental results demonstrate the flexibility, efficiency, and accessibility of LayoutCopilot in handling real-world analog designs.

==> doc/ack.tex <==
\section{Acknowledgement}
This work is supported in part by the National Science Foundation of China (Grant No. 62141404, 62125401, 62034007), the Natural Science Foundation of Beijing, China (Grant No. Z230002), STIC (Grant No. QYJS-2023-2303-B), and the 111 project (B18001).

==> doc/answer.tex <==
{
\onecolumn
\normalsize

\ \\
\textbf{Responses to the reviewers}

\ \\
\textbf{Reviewer 1}
\begin{description}\itemsep.8em
\item[R1C1]
  \textbf{
xxx
  }
\item[R1A1]
Thanks very much for the comments.

\item[R1C2]
  \textbf{
xxx
    }
\item[R1A2]
xxx
\end{description}

\ \\
}


==> doc/cover.tex <==
\twocolumn[
\begin{@twocolumnfalse}

Dear Editor and Reviewers,

% \ \\
% Thank you very much for reviewing our submission.

% \ \\
% We have revised our submission according to the reviewers' suggestions. All the changes are highlighted with \textcolor{blue}{blue} color.
 \\
Thank you for your letter and for the reviewers' comments concerning our manuscript entitled ``LayoutCopilot: An LLM-powered Multi-agent Collaborative Framework for Interactive Analog Layout Design''(lD: TCAD-2024-0651). Those comments are all valuable and very helpful for revising and improving our paper, as well as the important guiding significance to our research. We have studied comments carefully and have made corrections which we hope meet with approval. Revised portions are marked in red on the paper. The main corrections in the paper and the responses to the reviewer's comments are as follows:

% \\
Respond to the reviewers' comments:

% \\/
\large
\textbf{Reviewer 1:}
\normalsize

%  \\
1. \textbf{Response to comment:} xxx\\
\textbf{Response:} xxx \\ 

%  \\
2. \textbf{Response to comment:} xxx\\
\textbf{Response:} xxx


%  \\
\textbf{Reviewer 2:}

%  \\
1. \textbf{Response to comment:} \emph{What motivates the use of a multi-agent system over a single-agent system? Since the LLM is not fine-tuned, it is challenging to discern the differences between these systems. Could you elaborate on the distinct roles of the Classifier Agent and the Solution Adapter Agent, especially since the same LLM API is utilized?} \\ 
\textbf{Response: } 
This comment includes several questions, and we address them one by one: 
\begin{itemize}
    \item \emph{What motivates the use of a multi-agent system over a single-agent system?}  \\
    As mentioned in the second paragraph of Section III.A, a single-agent system does not perform well when dealing with diverse tasks. We believe this is due to what we call "prompt dilution," where prompts contain irrelevant information for a specific task, resulting in suboptimal performance. For example, if an LLM is instructed to handle tasks A, B, and C, and then asked to perform task A, its performance is likely to be inferior compared to a scenario where the LLM is only given instructions for task A. Our experiments support this, showing that the multi-agent system improves results by focusing more specifically on individual tasks.

    \item \emph{Since the LLM is not fine-tuned, it is challenging to discern the differences between these systems.}  \\
    While it is true that the LLM is not fine-tuned, fine-tuning is not the only method to enhance model performance. Prompt engineering plays a crucial role in shaping the behavior of the model. The LLM tends to perform better when given instructions tailored to a specific task, while for tasks unrelated to the instruction, the LLM might perform worse by attempting to follow the irrelevant parts of the instruction. In conclusion, the differences between the systems arise from the specific content passed in the prompts (which can also be referred to as instructions or system messages). As a result, even with the same LLM API, performance varies across different tasks.
    
    \item \emph{Could you elaborate on the distinct roles of the Classifier Agent and the Solution Adapter Agent, especially since the same LLM API is utilized?}  \\
    Additional clarifications have been provided in Sections III.A.3 and III.A.4, but due to space constraints, more detailed explanations are included below:
    \begin{itemize}
        \item The \textbf{Classifier Agent} is responsible for distinguishing whether a designer's request is concrete or abstract, which determines the subsequent workflow (whether it proceeds directly to task-specific processing). Since we cannot expect designers to always clearly specify this information in natural language inputs, the Classifier Agent handles this task. The instructions provided to the LLM include specific guidelines:
        \begin{itemize}
            \item \textbf{Concrete requests} contain explicit P\textbackslash\&R (Place \textbackslash\& Route) modification instructions with clear targets (e.g., devices) and parameters (e.g., coordinates, values).
            \item \textbf{Abstract requests} lack such clear information.
        \end{itemize}
        The Classifier Agent can access a command list, allowing it to determine whether the designer's instruction falls within the capabilities of the layout tool. If the request exceeds these capabilities, feedback is given directly to the designer. This feedback loop, not shown previously due to space limitations, will be added. Additionally, few-shot learning examples are provided to further ensure classification accuracy.
        \item The \textbf{Solution Adapter Agent} is responsible for converting refined solutions into concrete, actionable requests. Refined requests, such as "improve the symmetry of the differential pair" or "increase the width of the power net," often do not include device-specific information related to the netlist. The Solution Adapter Agent reads the netlist, identifies the specific devices or nets involved (e.g., identifying the MOSFETs in a differential pair or locating the power net), and rephrases the refined solutions to generate concrete requests that can be applied to the actual circuit. It also serves as a safeguard by cross-checking the command list of the layout tool to ensure that the generated concrete requests are executable within the tool’s capability, and to verify the completeness of their parameters.
    \end{itemize}
    Together, these two agents function as a filter for the Concrete Request Processor, ensuring that all requests entering the subsequent workflow are standardized and correctly processed.
\end{itemize}

%  \\
% 2. Response to comment: \\
% Response: xxx

%  \\
% Best regards,

%  \\

% Bingyang Liu ... \\

1. \textbf{Response to comment:} \emph{R1: 3. The comparison in Table IV is not fair. This is because symmetry constraint extraction is a key feature of MAGICAL, but the author used a version without any constraint, as shown in Fig.9(1).} \\ \emph{R3: 1. Introducing LLMs into the analog layout generation problem is worth exploring. However, the approach mainly shifts existing workflows from manual scripting to natural language commands, without significantly advancing the state of the art in layout design.} \\ \emph{R3: 5. LayoutCopilot does not significantly outperform existing tools like MAGICAL, particularly in
the comparator case. The limited number and small scale of the circuit cases further weaken
the paper's impact.} \\ 

\textbf{Response:} Actually, the LayoutCopilot is an LLM-powered framework based on interactive analog layout design tools. This approach is actually a semi-automated method that requires human involvement. The final layout performance depends on the experience of users. As Figure~\ref{interactive_result} shows, the layout after interactive adjustment can outperform the MAGICAL and can be further enhanced by more adjustment steps. Thus, the main purpose of LayoutCopilot is not to generate analog layouts automatically but to offer an efficient way to easily reach the manual layout designs. First, LayoutCopilot shows that the LLM is capable of translating natural language into domain-specific scripts with concise prompting(Concrete Experiments). Second, LayoutCopilot demonstrates that the LLM is capable of understanding analog designs and dramatically improving the layout performance (actually is as good as MAGICAL with constraint) compared to a raw automatic tool(Abstract Experiments). As the first work of LLM application in analog layout, this work mainly demonstrates the comprehension ability of LLM in analog designs. In future work, with more analog layout data we will fine-tune the large language model to exceed the traditional fully automated analog layout generators.

\end{@twocolumnfalse}
]






\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.48\linewidth]{figs/Interactive_result.png}
    \caption{Interactive results~\cite{gao_interactive_2023}.}
    \centering
    \label{interactive_result}
\end{figure*}


\clearpage




==> texlib/acm_setting.tex <==
% =============================================================
%            settign for ACM format paper
%
%   Author      : Bei Yu
%   Last Update : 12/2014
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
\geometry{twoside=true, head=13pt,
	paperwidth=8.5in, paperheight=11in,
	includeheadfoot, columnsep=2pc,
	top=35pt, bottom=45pt, 
    left=50pt, right=50pt, 
    %inner=54pt, outer=54pt,
	marginparwidth=2pc,heightrounded
}%
%\geometry{twoside=true, head=13pt,
%paperwidth=8.5in, paperheight=11in,
%includeheadfoot, columnsep=2pc,
%top=57pt, bottom=73pt, inner=54pt, outer=54pt,
%marginparwidth=2pc,heightrounded
%}%
\iffalse
\textfloatsep          = 12pt plus 1pt minus 7pt            % set space between figure and text
\floatsep              = 5pt plus 1pt minus 7pt
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{graphicx}
\usepackage{amsmath}
\let\Bbbk\relax
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{comment}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm}
\usepackage{multirow}
\usepackage{threeparttable,booktabs}
\usepackage{tikz}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{cleveref}                                      % smart citation
\usepackage[mathcal]{eucal}
%\usepackage[]{algpseudocode}                               % algorithm package
\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{siunitx}


\sisetup{product-units = single}
% ==== Local new commands
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
\newcommand{\m}[1]{\mathbf{#1}}
\newcommand{\mx}{\m{x}}
\newcommand{\my}{\m{y}}
\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}



% ==== spacing control on caption
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}


==> texlib/ieee_normal.tex <==
% =============================================================
%         setting for IEEE format paper (normal mode)
%
%   Author      : Bei Yu
%   Last Update : 09/2016
% =============================================================


%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}                                 % new algorithm package
\usepackage{algorithm}
\usepackage{graphicx}                                      % include pdf figures
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage[subrefformat=parens,farskip=0pt,justification=centering]{subfig}
\usepackage{color}
\usepackage{cite}                                          % more citations in one bracket
\usepackage{comment}                                       % use comment
\usepackage{soul}                                          % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}                                      % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}                                           % nth command
\usepackage{bm}                                            % bm command
\usepackage{courier}
\usepackage{balance}
\usepackage{threeparttable}
\usepackage[bookmarks=false]{hyperref}                     %
\hypersetup{
    colorlinks = true,
    citecolor  = blue,
    linkcolor  = blue,
    urlcolor   = blue,
}
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{caption} 
\captionsetup[table]{skip=4pt}
\setlength{\columnsep}{18pt}                               % set space between columns
\definecolor{CUHKorange}{RGB}{244,106,18} %F47012
\definecolor{CUHKblue}{RGB}{0,111,190}    %006FBE
\definecolor{CUHKgreen}{RGB}{0,127,128}   %007F80
\definecolor{CUHKred}{RGB}{228,46,36}     %E42E24
\definecolor{CUHKyellow}{RGB}{198,148,34} %C69422
\definecolor{CUHKdark}{RGB}{114,44,114}   %722C72
\definecolor{CUHKmiddle}{RGB}{144,44,144} %902C90
\definecolor{CUHKlight}{RGB}{167,44,167} 

% =============================================================
%                   Theorem Definitions
% =============================================================
% \newtheorem{myproblem}{\textbf{Problem}}
% \newtheorem{mydefinition}{\textbf{Definition}}
% \newtheorem{mytheorem}{\textbf{Theorem}}
% \newtheorem{mycorollary}{\textbf{Corollary}}
% \newtheorem{mylemma}{\textbf{Lemma}}
% \newtheorem{myclaim}{\textbf{Claim}}
% \newtheorem{myapplication}{\textbf{Application}}
% % \newtheorem{myconjecture}{Conjecture}
% \newtheorem{myprop}{Property}

\algrenewcommand\textproc{\texttt}
\newcommand{\tabincell}[2]{
    \begin{tabular}{@{}#1@{}}#2\end{tabular}
}

% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% =============================================================
%          Definitions to support latexdiff
% =============================================================
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}{#1}}}                           %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                       %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{}                                                   %DIF PREAMBLE
\providecommand{\DIFaddend}{}                                                     %DIF PREAMBLE
\providecommand{\DIFdelbegin}{}                                                   %DIF PREAMBLE
\providecommand{\DIFdelend}{}                                                     %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}                                        %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}                                        %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{}                                                 %DIF PREAMBLE
\providecommand{\DIFaddendFL}{}                                                   %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{}                                                 %DIF PREAMBLE
\providecommand{\DIFdelendFL}{}                                                   %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF


% ==== Logs:
%
%  09/2016: captionsetup, columnsep
%  07/2016: support to pgfplots
%  07/2016: threeparttable
%  04/2016: definitions supporting latexdiff
%  04/2016: remove bookmarks in hyperref
%  02/2016: tabincell
%  02/2016: hyperref
%  12/2015: copy from "ieee_conference"
%



==> texlib/poster_setting.tex <==
% ============================================================
%             Beamer poster setting file
%
%   Author      : Bei Yu
%   last Update : 06/2014
% ============================================================

% additional settings
\setbeamerfont{itemize}{size=\normalsize}
\setbeamerfont{itemize/enumerate body}{size=\normalsize}
\setbeamerfont{itemize/enumerate subbody}{size=\normalsize}


% block width setting
\newenvironment<>{varblock}[2][\textwidth]{%
  \setlength{\textwidth}{#1}
  \setbeamercolor{block title}{fg=white,bg=blue!20!green}
  %\setbeamercolor{block body}{fg=black,bg=olive!50}
  \setbeamercolor{block body}{fg=black,bg=blue!10}
  \begin{actionenv}#3%
  \def\insertblocktitle{#2}%
  \par%
  \usebeamertemplate{block begin}}
  {
    \par%
    \usebeamertemplate{block end}%
    \end{actionenv}
  }


% abbreviations
\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{{etc}\onedot}
\def\vs{{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\etal{{et al}\onedot}
\makeatother


% === including packages
\usepackage{bm}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{times}
\usepackage{amsmath,amsthm, amssymb, latexsym}
\usepackage{exscale}
\usepackage{subfigure}
\usepackage{multirow}
\usepackage{comment}
\usepackage{booktabs, array}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage[orientation=landscape,size=custom,width=200,height=230,scale=1.9]{beamerposter}
\listfiles

% =====  algorithm setting
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}
\usepackage{algorithm}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
%\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm

% ==== Log
%
%  05/2014: preliminary results show that pgf library is NOT good for poster
%


